REMONI: An Autonomous System Integrating Wearables and Multimodal Large Language Models for Enhanced Remote Health Monitoring

With the widespread adoption of wearable devices in our daily lives, the demand and appeal for remote patient monitoring have significantly increased. Most research in this field has concentrated on collecting sensor data, visualizing it, and analyzing it to detect anomalies in specific diseases such as diabetes, heart disease and depression. However, this domain has a notable gap in the aspect of human-machine interaction. This paper proposes REMONI, an autonomous REmote health MONItoring system that integrates multimodal large language models (MLLMs), the Internet of Things (IoT), and wearable devices. The system automatically and continuously collects vital signs, accelerometer data from a special wearable (such as a smartwatch), and visual data in patient video clips collected from cameras. This data is processed by an anomaly detection module, which includes a fall detection model and algorithms to identify and alert caregivers of the patient's emergency conditions. A distinctive feature of our proposed system is the natural language processing component, developed with MLLMs capable of detecting and recognizing a patient's activity and emotion while responding to healthcare worker's inquiries. Additionally, prompt engineering is employed to integrate all patient information seamlessly. As a result, doctors and nurses can access real-time vital signs and the patient's current state and mood by interacting with an intelligent agent through a user-friendly web application. Our experiments demonstrate that our system is implementable and scalable for real-life scenarios, potentially reducing the workload of medical professionals and healthcare costs. A full-fledged prototype illustrating the functionalities of the system has been developed and being tested to demonstrate the robustness of its various capabilities.

==> TikzPlotLib/loss.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}

\begin{groupplot}[group style={group size=1 by 2}]
\nextgroupplot[
axis line style={lightgray204},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
%title={Training and Validation Loss},
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{Epochs},
xmajorgrids,
xmajorticks=true,
xmin=0, xmax=40,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{Loss},
ymajorgrids,
ymajorticks=true,
ymin=0, ymax=0.60,
ytick style={color=darkslategray38}
]
\addplot [thick, mediumseagreen85168104, dashed]
table {%
0 0.602986872196198
1 0.497753977775574
2 0.378174006938934
3 0.302105009555817
4 0.210285365581512
5 0.210732996463776
6 0.167035520076752
7 0.188879564404488
8 0.138329312205315
9 0.131013989448547
10 0.11280120164156
11 0.0859636589884758
12 0.0744747370481491
13 0.102660246193409
14 0.0690149068832397
15 0.0680183693766594
16 0.0616145990788937
17 0.0623553022742271
18 0.0446868985891342
19 0.0350649952888489
20 0.0254171658307314
21 0.0266014151275158
22 0.0240923818200827
23 0.0252497810870409
24 0.0214814487844706
25 0.0190167967230082
26 0.0181898567825556
27 0.0171282086521387
28 0.0177738126367331
29 0.0170745756477118
30 0.0173876639455557
31 0.0185067411512136
32 0.0194836780428886
33 0.0200204718858004
34 0.0271972641348839
35 0.0175135899335146
36 0.019660348072648
37 0.0198304448276758
38 0.0192056931555271
39 0.0182619132101536
};
\addlegendentry{Training Loss}
\addplot [thick, mediumseagreen85168104]
table {%
0 0.516670703887939
1 0.45409682393074
2 0.420059740543365
3 0.364117205142975
4 0.332244336605072
5 0.227987140417099
6 0.316742122173309
7 0.292347073554993
8 0.246449410915375
9 0.207891672849655
10 0.224702149629593
11 0.193555161356926
12 0.250982344150543
13 0.198463156819344
14 0.221531480550766
15 0.28878653049469
16 0.287453591823578
17 0.199796319007874
18 0.191396474838257
19 0.186330199241638
20 0.18885563313961
21 0.190470308065414
22 0.18941655755043
23 0.193533658981323
24 0.190385609865189
25 0.190668880939484
26 0.190988272428513
27 0.190776348114014
28 0.190969407558441
29 0.191141530871391
30 0.191114574670792
31 0.191162690520287
32 0.191265016794205
33 0.191351175308228
34 0.191358149051666
35 0.191364124417305
36 0.191375032067299
37 0.191380798816681
38 0.191379532217979
39 0.191390812397003
};
\addlegendentry{Validation Loss}
\end{groupplot}

\end{tikzpicture}

